ContraDoc: Understanding Self-Contradictions in Documents with Large Language Models

In recent times, large language models (LLMs) have shown impressive performance on various document-level tasks such as document classification, summarization, and question-answering. However, research on understanding their capabilities on the task of self-contradictions in long documents has been very limited. In this work, we introduce ContraDoc, the first human-annotated dataset to study self-contradictions in long documents across multiple domains, varying document lengths, self-contradictions types, and scope. We then analyze the current capabilities of four state-of-the-art open-source and commercially available LLMs: GPT3.5, GPT4, PaLM2, and LLaMAv2 on this dataset. While GPT4 performs the best and can outperform humans on this task, we find that it is still unreliable and struggles with self-contradictions that require more nuance and context. We release the dataset and all the code associated with the experiments (https://github.com/ddhruvkr/CONTRADOC).

==> responsibleNLPresearch.tex <==
%-----------------------------------------------------------------------------------
% Responsible NLP research checklist version 0.1
% 
% This checklist was created by Marine Carpuat, Marie-Catherine de Marneffe and Ivan Vladimir Meza Ruiz,
% the NAACL 2022 program chairs, working with Jesse Dodge and the ARR editors-in-chief Pascale Fung,
% Goran Glavas, Sebastian Riedel and Amanda Stent. Source updated by Vilém Zouhar.
% Additional feedback was provided by Anna Rogers, Margot Mieskes and the NAACL 2022 reproducibility chairs.
% The checklist was reviewed by the ACL Ethics Committee.
% 
% Subject to change.
%------------------------------------------------------------------------------------



% Command for choice menu 
\newcommand{\cm}[3]{\mbox{\ChoiceMenu[height=0.3cm,width=0.3cm,bordercolor=,name=#1,radio,radiosymbol=\ding{108},default=#3]{}{#2}}}

% Command for text field
\newcommand{\tf}[3][0.78]{\mbox{\TextField[bordercolor=,name=#2,value={#3},multiline=true,height=4em, width=#1\textwidth]{\noindent \parbox{0.11\textwidth}{Section or\\Justification}}}}

% Command for checkbox
\newcommand{\cb}[1]{\mbox{\CheckBox[bordercolor=,name=#1,height=0.4cm,width=0.4cm]{}{\ }}}

% Fix choice menu
\makeatletter
    \patchcmd{\HyField@FlagsRadioButton}{\HyField@SetFlag{Ff}{Radio}}{}{}{}
\makeatother

\titleformat{\section}{\Large\bfseries}{\Alph{section}}{1em}{}
\titleformat{\subsection}{\normalfont\bfseries}{\Alph{section}\arabic{subsection}}{1em}{}

\title{Responsible NLP Research Checklist\vspace{-3em}}
\date{}

\begin{document}
\maketitle

Members of the ACL are responsible for adhering to the \href{https://www.aclweb.org/portal/content/acl-code-ethics}{ACL code of ethics}. The ARR Responsible NLP Research checklist is designed to encourage best practices for responsible research, addressing issues of research ethics, societal impact and reproducibility.

Please read the \href{https://aclrollingreview.org/responsibleNLPresearch/}{Responsible NLP Research checklist guidelines} for information on how to answer these questions. Note that not answering positively to a question is not grounds for rejection. 

All supporting evidence can appear either in the main paper or the supplemental material. For each question, if you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification.

Please do \textbf{not} modify, reorder, delete or add questions, question options or other wording of this document.

% USAGE:
% Use the last argument in the \cm and \tf commands to mark your answer, e.g.:
% \cm{mainClaims}{Yes,No,N/A}{N/A}
% \tf[0.85]{mainClaimsJustification}{This does not apply...}

\section{For every submission}

\subsection{Did you discuss the \textit{limitations} of your work?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{mainClaims}{Yes,No,N/A}{}\\[0.2cm]
    \tf[0.85]{mainClaimsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]
        
\subsection{Did you discuss any potential \textit{risks} of your work?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{risks}{Yes,No,N/A}{}\\[0.2cm]
    \tf[0.85]{risksJustification}{}
\end{tabular}
\end{Form}

\subsection{Do the abstract and introduction summarize the paper’s main claims?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{abstractIntro}{Yes,No,N/A}{}\\[0.2cm]
    \tf[0.85]{abstractIntroJustification}{}
\end{tabular}
\end{Form}

\section{Did you use or create \textit{scientific artifacts}?}
If you answer {\bf Yes}, answer the questions below; if you answer {\bf No}, you can skip the rest of this section. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
\cm{createArtifacts}{Yes,No}{}\\[0.2cm]
\end{tabular}
\end{Form}

If yes:
\subsection{Did you cite the creators of artifacts you used?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
   \begin{tabular}{l}
    \cm{citeCreators}{Yes,No,N/A}{}\\[0.2cm]
    \tf{citeCreatorsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss the \textit{license or terms} for use and/or distribution of any artifacts?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
   \begin{tabular}{l}
    \cm{legalGrounds}{Yes,No,N/A}{}\\[0.2cm]
    \tf{legalGroundsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss if your use of existing artifact(s) was consistent with their \textit{intended use}, provided that it was specified? For the artifacts you create, do you specify intended use and whether that is compatible with the original access conditions (in particular, derivatives of data accessed for research purposes should not be used outside of research contexts)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
   \begin{tabular}{l}
    \cm{intendedUse}{Yes,No,N/A}{}\\[0.2cm]
    \tf{intendedUseJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss the steps taken to check whether the data that was collected/used contains any \textit{information that names or uniquely identifies individual people} or \textit{offensive content}, and the steps taken to protect / anonymize it?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{personallyIdentifiableInformationOrOffensiveContent}{Yes,No,N/A}{}\\[0.2cm]
    \tf{personallyIdentifiableInformationOrOffensiveContentJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you provide documentation of the artifacts, e.g., coverage of domains, languages, and linguistic phenomena, demographic groups represented, etc.?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{documentation}{Yes,No,N/A}{}\\[0.2cm]
    \tf{documentationJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report relevant statistics like the number of examples, details of train/test/dev splits, etc. for the data that you used/created?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{relevantStatistics}{Yes,No,N/A}{}\\[0.2cm]
    \tf{relevantStatisticsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\section{Did you run \textit{computational experiments}?} 
If you answer {\bf Yes}, answer the questions below; if you answer {\bf No}, you can skip the rest of this section. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{computationalExperiments}{Yes,No}{}
\end{tabular}
\end{Form}

If yes:
\subsection{Did you report the \textit{number of parameters} in the models used, the \textit{total computational budget} (e.g., GPU hours), and \textit{computing infrastructure} used?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{reportReproducibility}{Yes,No,N/A}{}\\[0.2cm]
    \tf{reportReproducibilityJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss the experimental setup, including \textit{hyperparameter search} and \textit{best-found hyperparameter} values?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{bestFoundHyperparameter}{Yes,No,N/A}{}\\[0.2cm]
    \tf{bestFoundHyperparameterJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report \textit{descriptive statistics} about your results (e.g., error bars around results, summary statistics from sets of experiments), and is it transparent whether you are reporting the max, mean, etc. or just a single run?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{descriptiveStatistics}{Yes,No,N/A}{}\\[0.2cm]
    \tf{descriptiveStatisticsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{If you used existing packages (e.g., for preprocessing, for normalization, or for evaluation), did you report the implementation, model, and parameter settings used (e.g., NLTK, Spacy, ROUGE, etc.)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{existingPackages}{Yes,No,N/A}{}\\[0.2cm]
    \tf{existingPackagesJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\section{Did you use \textit{human annotators} (e.g., crowdworkers) or \textit{research with human subjects}?}
If you answer {\bf Yes}, answer the questions below; if you answer {\bf No}, you can skip the rest of this section. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{hummanAnnotators}{Yes,No}{}\\
\end{tabular}
\end{Form}

If yes:
\subsection{Did you report the full text of instructions given to participants, including e.g., screenshots, disclaimers of any risks to participants or annotators, etc.?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{fullTextInstructions}{Yes,No,N/A}{}\\[0.2cm]
    \tf{fullTextInstructionsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report information about how you recruited (e.g., crowdsourcing platform, students) and paid participants, and discuss if such \textit{payment is adequate} given the participants’ demographic (e.g., country of residence)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{payment}{Yes,No,N/A}{}\\[0.2cm]
    \tf{paymentJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss whether and how \textit{consent} was obtained from people whose data you're using/curating (e.g., did your instructions explain how the data would be used)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{consent}{Yes,No,N/A}{}\\[0.2cm]
    \tf{consentJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Was the data collection protocol \textit{approved (or determined exempt)} by an ethics review board?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{ethicsAmountSpent}{Yes,No,N/A}{}\\[0.2cm]
    \tf{ethicsAmountSpentJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report the basic demographic and geographic characteristics of the \textit{annotator} population that is the source of the data?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{annotator}{Yes,No,N/A}{}\\[0.2cm]
    \tf{annotatorJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\section{Did you use \textit{AI assistants} (e.g., ChatGPT, Copilot) in your research, coding, or writing?}
If you answer {\bf Yes}, answer the question below; if you answer {\bf No}, you can skip the rest of this section. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{aiAssistants}{Yes,No}{}\\
\end{tabular}
\end{Form}

\subsection{Did you include information about your use of AI assistants?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{aiAssistantsInformation}{Yes,No,N/A}{}\\[0.2cm]
    \tf{aiAssistantsInformationJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\end{document}


==> tab/dataset_statistics.tex <==
\begin{table}[]
    \centering
    \small
    \begin{tabular}{l|c|c} 
     \toprule
     \textbf{Categories} & \textbf{Attributes} & \textbf{\# docs} \\ 
    \midrule
    \multirow{3}{*}{\textbf{Document Type}} & \makecell[tl]{News\\Wikipedia\\Story} & \makecell[tl]{158\\150\\141} \\
     \midrule
     %\multirow{2}{*}{\textsc{Type}} & \makecell[tl]{positive\\negative} & \makecell[tl]{449 \\450} \\
     %\midrule
    
     \multirow{4}{*}{\shortstack[l]{\textbf{Document}\\\textbf{Length (tokens)}}} & \makecell[tl]{100-500\\500-1000\\1000-1500\\1500-2200} & \makecell[tl]{50\\184\\143\\72} \\
     \midrule
     \multirow{3}{*}{\shortstack[l]{\textbf{Self-Contradiction}\\\textbf{Range}}} & \makecell[tl]{global\\local\\intra} & \makecell[tl]{155 \\220\\73} \\
    \midrule
    \multirow{8}{*}{\shortstack[l]{\textbf{Self-Contradiction}\\\textbf{Type}}} & \makecell[tl]{Negation \\Numeric\\Content\\Perspective/View/Opinion\\Emotion/Mood/Feeling\\Factual\\Relation\\Causal} & \makecell[tl]{87\\66\\288\\101\\86\\54\\25\\36} \\
    %\midrule
    %\multirow{2}{*}{Contradiction Create} & \makecell[tl]{Replace\\Insert} & \makecell[tl]{271 \\178} \\
     \bottomrule
    \end{tabular}
    \caption{Breakdown of documents by different categories in \datapos (i.e. containing self-contradictions).}
    \label{tab:dataset_statistic}
\end{table}


==> tab/fine_grained_human.tex <==
\begin{table*}
\centering
\small
  \begin{tabular}{|c|l|l|l|l|l|l|l|l}
    \hline
    \multirow{2}{*}{Axis} &
    \multirow{2}{*}{Sub Axis} &
    \multirow{2}{*}{Total cases} &
    \multicolumn{2}{c}{Human} &
    \multicolumn{2}{c}{GPT3.5} &
    \multicolumn{2}{c}{GPT4} \\
    \cmidrule(lr){4-9} &
    \tiny{} & \tiny{} & \tiny{Found Cases} & \tiny{Accuracy} & \tiny{Found Cases} & \tiny{Accuracy} &  \tiny{Found Cases} & \tiny{Accuracy} \\
    \hline
    \multirow{3}{*}{\textsc{Range}} & \makecell[tl]{global \\local\\intra} & \makecell[tl]{155\\220\\73} & \makecell[tl]{79\\85\\27} & \makecell[tl]{0.51 \\0.39\\0.37} & \makecell[tl]{79\\85\\27} & \makecell[tl]{0.51 \\0.39\\0.37}& \makecell[tl]{138\\139\\37} & \makecell[tl]{0.89\\0.63\\0.51} \\
    \hline
  \end{tabular}
  \caption{Fine-grained performance analysis of humans and LLMs on top-k evidence selection.}
\label{tab:fine_grained_human}
\end{table*}





==> tab/prompt3_copy.tex <==
\begin{table*}
\centering
\small
  \begin{tabular}{|p{0.08\linewidth}|p{0.08\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.1\linewidth}}
    \hline
    \textbf{Dataset} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} &  \textbf{Accuracy (before verification)} & \textbf{Accuracy (after verification)} & \textbf{TP Rate} & \textbf{FP Rate} & \textbf{TN Rate} & \textbf{FN Rate} & \textbf{TP Success Verify}\\
    \hline
    ChatGPT & 57.48\% & 61.62\% & 40.94\% & 49.19\% & 45.3\% & 20.6\% & 12.8\% & 36.9\% & 29.7\% & 40.98 \\
    GPT4 & 88\% & 39.4\% & 54.5\% & 66.78\% & 65.32\% & 19.6\% & 2.65\% & 46.24\% & 31.5\% & 92.7\% \\
    PaLM2 & 52.5\% & 82.6\% & 64.2\% & 53.6\% & 29.0\% & 41.5\% & 37.6\% & 12\% & 9\% & 41\% \\
    Llama2 70b & 49.7\% & 95.5\% & 65.4\% & 49.16\% & 8.1\% & 48.03\% & 48.6\% & 1.12\% & 2.25\%& 14.5\%  \\
    \hline
  \end{tabular}
  \caption{Performance comparison of different LLMs on Prompt 3. Precision, Recall, F1 scores are values based on the "Yes/No" prediction on the entire dataset. Accuracy(before verification) is the percentage of correct prediction of "Yes/No" on the entire dataset. Accuracy (after verification) is the percentage of correct prediction of "Yes/No" after the evidence was evaluated. TP, FP, TN, and FN rates are calculated on the entire dataset before verification, i.e. on "Yes/No" prediction. TP (after verification) is the TP value after the evidence is evaluated.}
\label{tab:prompt3_copy}
\end{table*}




